Tidal interactions between binary stars drives lithium production in low-mass red giants

Theoretical models of stellar evolution predict that most of the lithium inside a star is destroyed as the star becomes a red giant. However, observations reveal that about 1% of red giants are peculiarly rich in lithium, often exceeding the amount in the interstellar medium or predicted from the Big Bang. With only about 150 lithium-rich giants discovered in the past four decades, and no distinguishing properties other than lithium enhancement, the origin of lithium-rich giant stars is one of the oldest problems in stellar astrophysics. Here we report the discovery of 2,330 low-mass (1 to 3$\,M_\odot$) lithium-rich giant stars, which we argue are consistent with internal lithium production that is driven by tidal spin-up by a binary companion. Our sample reveals that most lithium-rich giants have helium-burning cores ($80^{+7}_{-6}\%$), and that the frequency of lithium-rich giants rises with increasing stellar metallicity. We find that while planet accretion may explain some lithium-rich giants, it cannot account for the majority that have helium-burning cores. We rule out most other proposed explanations as the primary mechanism for lithium-rich giants, including all stages related to single star evolution. Our analysis shows that giants remain lithium-rich for only about two million years. A prediction from this lithium depletion timescale is that most lithium-rich giants with a helium-burning core have a binary companion.

==> Makefile <==
.PHONY : clean, default, publish

REPO_NAME   = $(echo $TRAVIS_REPO_SLUG | cut -f2 -d/) 
TEX_FILES   = eneloop
TMP_SUFFS   = pdf aux bbl blg log dvi ps eps out ent
LATEX       = pdflatex -interaction=nonstopmode -halt-on-error
SUFF        = pdf
RM_TMP      = $(foreach d, ${TEX_FILES}, rm -rf $(foreach suff, ${TMP_SUFFS}, ${d}.${suff})) eneloopNotes.bib
CHECK_RERUN = grep Rerun eneloop.log
FIGURES     = $(patsubst %.py,%.pdf,$(wildcard figures/*.py))
TECTONIC    = $(shell command -v tectonic >/dev/null && echo true || echo false )

default: eneloop.pdf

eneloop.pdf: eneloop.tex eneloop.bib $(FIGURES)
	# Generate links to current git commit
	#python gen_links.py
	# Compile the paper with either tectonic or pdflatex
	if [ "${TECTONIC}" = "true" ]; then\
		tectonic eneloop.tex --print --keep-logs;\
	else\
		${LATEX} eneloop.tex;\
		( ${CHECK_RERUN} && bibtex eneloop.tex ) || echo "Done.";\
		( ${CHECK_RERUN} && ${LATEX} eneloop.tex ) || echo "Done.";\
		( ${CHECK_RERUN} && ${LATEX} eneloop.tex ) || echo "Done.";\
	fi

clean:
	# Remove temporaries and output
	$(RM_TMP)
	rm -rf $(FIGURES)

figures/%.pdf: figures/%.py
	# Generate all figures
	cd $(<D);python $(<F)

